Outage-Watch: Early Prediction of Outages using Extreme Event Regularizer

Cloud services are omnipresent and critical cloud service failure is a fact of life. In order to retain customers and prevent revenue loss, it is important to provide high reliability guarantees for these services. One way to do this is by predicting outages in advance, which can help in reducing the severity as well as time to recovery. It is difficult to forecast critical failures due to the rarity of these events. Moreover, critical failures are ill-defined in terms of observable data. Our proposed method, Outage-Watch, defines critical service outages as deteriorations in the Quality of Service (QoS) captured by a set of metrics. Outage-Watch detects such outages in advance by using current system state to predict whether the QoS metrics will cross a threshold and initiate an extreme event. A mixture of Gaussian is used to model the distribution of the QoS metrics for flexibility and an extreme event regularizer helps in improving learning in tail of the distribution. An outage is predicted if the probability of any one of the QoS metrics crossing threshold changes significantly. Our evaluation on a real-world SaaS company dataset shows that Outage-Watch significantly outperforms traditional methods with an average AUC of 0.98. Additionally, Outage-Watch detects all the outages exhibiting a change in service metrics and reduces the Mean Time To Detection (MTTD) of outages by up to 88% when deployed in an enterprise cloud-service system, demonstrating efficacy of our proposed method.

==> tex/07.Data.tex <==
\section{Data Generation} \label{sec:data_gen}

\subsubsection{Alerts Data}
We have fetched alert occurrence data for Adobe Sign from PagerDuty\footnote{\href{https://www.pagerduty.com/}{https://www.pagerduty.com/}} between the dates from October 2020 to June 2022, which included a total of $\sim44,000$ alerts logged through 13 monitors. Out of these, $\sim940$ unique alerts were fired over the entire time period. 

\subsubsection{CSO Reports} \label{sec:data-cso}
CSO post-mortem reports of Adobe Sign service were fetched from October 2018 to June 2022 from the CSO Executive Dashboard\footnote{\href{https://app.powerbi.com/groups/me/apps/fee6a203-c7e7-4d5c-bf16-830541fdc5c5/reports/68c84e63-95f4-47c7-9dbc-b941259ba578/ReportSectione08467a22d1931c8e0ee}{CSO Executive Dashboard}}. It included a total of 182 reports, where each report has information on the symptoms of the outage, its impact, the root cause and the remediation strategies involved in ameliorating the effects of the outage. Additionally, information on the affected services, CSO duration and related incidents are also mentioned. 

